BenchQC -- Scalable and modular benchmarking of industrial quantum computing applications

We present BenchQC, a research project funded by the state of Bavaria, which promotes an application-centric perspective for benchmarking real-world quantum applications. Diverse use cases from industry consortium members are the starting point of a benchmarking workflow, that builds on the open-source platform QUARK, encompassing the full quantum software stack from the hardware provider interface to the application layer. By identifying and evaluating key metrics across the entire pipeline, we aim to uncover meaningful trends, provide systematic guidance on quantum utility, and distinguish promising research directions from less viable approaches. Ultimately, this initiative contributes to the broader effort of establishing reliable benchmarking standards that drive the transition from experimental demonstrations to practical quantum advantage.

==> sections/objectives.tex <==
\subsection{Consortium}
% \todo[inline]{
% BMW, Reply, Optware, Quantinuum, Fraunhofer IIS, Fraunhofer IKS
% }

The \textbf{Fraunhofer Institute for Cognitive Systems IKS} focuses on the field of safe artificial intelligence and safe software engineering to enable the use of these technologies in safety-critical areas. It has vast experience in the development of reliable AI applications for markets such as autonomous driving, industry 4.0, or healthcare. In the quantum computing domain, Fraunhofer IKS is researching on how to enable robust and reliable applications of quantum computing, such that this new technology can be used in safety-critical areas. In terms of application scenarios, the Fraunhofer IKS mainly considers challenges in optimization and quantum-enhanced machine learning, as e.g., using quantum computing for medical imaging. It also leads the application consortium in the Munich Quantum Valley.


The \textbf{Fraunhofer Institute for Integrated Circuits IIS} is a leader in international research for microelectronic and information technology solutions and services. It has extensive experience in transferring new algorithmic technologies from fundamental research to application, now expanding its focus to QC and quantum algorithms. The institute is active in various projects for mathematical optimization and quantum machine learning, including the research of potential of QC-supported reinforcement learning in collaboration with industry partners.

\textbf{Machine Learning Reply} began exploring practical applications of quantum computing in 2018 and has implemented over 20 proof-of-concept use cases across various industries. This resulted for example in the development of an efficient classical solver for QUBO problems. ML Reply won the Airbus Quantum Computing Challenge in 2020 and reached the finals of the BMW/AWS Quantum Computing Challenge in 2021, aiming to solidify its hands-on experience through research projects.

The \textbf{OptWare GmbH} has been designing and implementing optimization and analytics in production and logistics systems for over 25 years, providing high-performance mathematical solutions for complex industry problems. The company uses AI/ML to uncover complex relationships and develops hybrid self-learning solutions that combine AI and optimization. In 2020, OptWare established an internal research group to evaluate the potential of quantum computing for its business, conducting practical studies in ongoing projects, supported by federal funding.

Vehicles are among the most complex consumer goods, with optimization potentials throughout the entire automotive value chain, particularly in production and logistics. The \textbf{BMW Group} recognized the potential of quantum computing in 2018 and established a dedicated QC team, which has since been an active member in the quantum ecosystem and was a co-founder of the Quantum Technology \& Application Consortium (QUTAC)~\cite{bayerstadler_industry_2021}. The company aims to identify when specific problem classes can benefit from quantum advantages and to translate technical advancements into business processes, addressing a key challenge for industrializing this technology.

\textbf{Quantinuum}, established through a merger of Honeywell Quantum Solutions and Cambridge Quantum Computing in 2021, builds trapped-ion quantum computers, as well as quantum software and algorithms in areas such as quantum chemistry, artificial intelligence, and quantum simulation. 
As of September 2024, Quantinuum's H2 quantum computer holds the world record in quantum volume at $2^{21}$.



\subsection{Motivation}
% \todo[inline]{
% TODO: cite economic gain of QC~\cite{jean-francois_bobier_what_2021}
% Motivate from real problems (BMW: QML, Optware, Reply)
% OptWare:
% \begin{itemize}
%  \item Maybe best use Motivation of project draft? 
%  \item Attention should be payed to Machine-Learning, Optimization and Simulation (all the fields of bench-qc). 
%  \item Emerging Technology $\Rightarrow$ Benchmarking to have tool ready as soon as break through takes place.
% \end{itemize}
% }
% \todo{Real use case examples Daria, Johannes. Mention challenges and reasons to have a project like BenchQC.}

Quantum computing has the potential to boost industrial applications in particular for optimization, simulation, and machine learning by solving problems that are currently intractable for classical systems, or by building more efficient solutions for already tractable problems, for example using less learning data.
The Boston Consulting Group estimates that, at tech maturity, quantum computing will unlock hundreds of use cases, with potential value creation of $\$100 B$ and more in \textit{each} of the above fields~\cite{jean-francois_bobier_what_2021}.
Being at the forefront of this emerging technology is therefore a competitive advantage that elicits strategic investments across various industrial domains. Problem instances studied in the BenchQC project range hereby from the optimal distribution and configuration of LiDAR sensors within production plants, over 6G beam management, to the simulation of dynamic fermions in material science (see Sec.~\ref{sec:usecases_opt}-\ref{sec:usecases_sim} for details). 
%One example that is evaluated in Bench-QC is the optimal distribution and configuration of LiDAR sensors within production plants. These sensors are used to provide real-time information about the surroundings of vehicles that drive autonomously from the end of the production line to the distribution area outside~\cite{BMW_AFW}. The goal of the underlying optimization problem is to minimize the number of sensors while providing coverage of the entire critical area of operation, leading to significant efficiency gains, cost savings, and improved overall productivity.

For company end users, however, it can be challenging to understand whether their problem category is well-suited to benefit from future quantum technology, how large the problem can be scaled, or which hardware and algorithms are the best fit.
%Industry is always looking for competitive advantages through the introduction of new technologies.  However, in order to make strategic investment decisions, companies need to assess when quantum technology will be ready for real use, how large the problems can be scaled, and which hardware and algorithms are best suited to their needs.
Benchmarking is crucial in this process, providing insight into the practical applicability of quantum solutions. It allows industrial players to track performance improvements, evaluate the scalability of quantum approaches, and ensure that tools are ready when breakthroughs occur. This is particularly important for companies dealing with complex and large use cases.
A strong benchmarking framework guides investment decisions and sets realistic expectations. Early involvement in benchmarking initiatives, for example, by actively exploring these technologies through small industry-based use cases, will allow industry to capitalize on advances in quantum technology as the technology becomes more mature. 

%\todo[inline]{move to optimization section (\ref{sec:Optimization})}
%Quantum computing has the potential to boost the efficiency of production processes, e.g., in the automotive industry by leveraging its ability to rapidly evaluate large-scale, complex scenarios and identify optimal solutions. 

% \subsection{Unique selling points}
% \begin{itemize}
% \item QML: Benchmarking for QML is less explored, theoretical guarantees for QML advantage are less clear, need for empirical benchmarking to give guidance about usability.
% \item Full stack approach: Have all components from hardware to software within the MQV
% \item Hardware diversity: MQV provides diverse quantum hardware for representative benchmarking
% \item Metrics: holistic view on metrics, little explored for QML
% \item Scalability: Various concepts to simulate problem complexity scaling (noise, modular scalable network size, etc.)
% \item Tooling: Tool compatibility within the MQV (MQT Bench, Optimization decision tree)?
% \end{itemize}


% \subsection{Work packages and structure}
% The work packages in the \textit{BenchQC} project are organized in the following structure:
% \begin{enumerate}
%     \item \textbf{Problem category analysis} (machine learning, simulation, optimization)
%     \begin{enumerate}
%         \item Metrics
%         \item Problem sequence scaling
%         \item Solution methods
%         \item Mapping
%         \item Benchmarking/potential analysis
%     \end{enumerate}
%     % \item Problem category simulation
%     % \item Problem category optimization
%     \item \textbf{Platform development}
%     \begin{enumerate}
%         \item Requirements analysis
%         \item Architecture design
%         \item Implementation
%     \end{enumerate}
%     \item \textbf{Use cases} (machine learning, simulation, optimization)
% \end{enumerate}

% The problem category analysis encompasses work items that include the selection of relevant metrics for a given application, as well as a variation of the problem scaling, to eventually map methods to existing hardware systems and benchmark candidate solutions. More details about individual steps are outlined in Sec.~\ref{sec:methodology}. The platform development work package is centered around the QUARK tool as described in Sec.~\ref{sec:tools}, which also includes interfaces to quantum hardware systems. The use cases section involves phrasing and implementing algorithmic solutions for relevant applications. Selected examples are discussed in Sec.~ \ref{sec:usecases_opt}-\ref{sec:usecases_sim}.
